ATLASGAL-selected massive clumps in the inner Galaxy, II: Characterisation of different evolutionary stages and their SiO emission

The processes leading to the birth of high-mass stars are poorly understood. We characterise here a sample of 430 massive clumps from the ATLASGAL survey, which are representative of different evolutionary stages. To establish a census of molecular tracers of their evolution we performed an unbiased spectral line survey covering the 3-mm atmospheric window between 84-117 GHz with the IRAM 30m. A smaller sample of 128 clumps has been observed in the SiO (5-4) transition with the APEX telescope to complement the SiO (2-1) line and probe the excitation conditions of the emitting gas, which is the main focus of the current study. We report a high detection rate of >75% of the SiO (2-1) line and a >90% detection rate from the dedicated follow-ups in the (5-4) transition. The SiO (2-1) line with broad line profiles and high detection rates, is a powerful probe of star formation activity, while the ubiquitous detection of SiO in all evolutionary stages suggests a continuous star formation process in massive clumps. We find a large fraction of infrared-quiet clumps to exhibit SiO emission, the majority of them only showing a low-velocity component (FWHM~5-6 km/s) centred at the rest velocity of the clump. In the current picture, where this is attributed to low-velocity shocks from cloud-cloud collisions, this can be used to pinpoint the youngest, thus, likely prestellar massive structures. Based on the line ratio of the (5-4) to the (2-1) line, our study reveals a trend of changing excitation conditions that lead to brighter emission in the (5-4) line towards more evolved sources. Our analysis delivers a more robust estimate of SiO column density and abundance than previous studies and questions the decrease of jet activity in massive clumps as a function of age.

==> SIO_LINEPARAMS.tex <==
%______________________________________________
\begin{table*}
\caption{SiO ($2-1$) line parameters and column density.}\label{tab:table-large-sio21}
\begin{center}
\begin{tabular}{lrrrrrrrrrrr}
\hline\hline
Source name\tablefootmark{a} & Ra    & Dec     &  $v_{\rm lsr}\tablefootmark{b}$& $\Delta v$\tablefootmark{c} &$\int$T$_{mb}\,\rm dv$ & $\sigma_{21}$\tablefootmark{d}& Wings &  $N(\rm{SiO})$ \tablefootmark{e}\\
            & J2000 [$^\circ$] & J2000 [$^\circ$]  &  [km/s] &  [km/s] &[K km/s]  & [K km/s] & & $\times10^{12}$ [cm$^{-2}$] \\
\hline
G06.22-0.61   &  270.5120   &    -23.8869   &   18.46   &  [    0.;   27.] &    2.84   &    0.25   &  y   &  5.08  \\
G08.68-0.37   &  271.5974   &    -21.6189   &   38.03   &  [   32.;   54.] &    8.68   &    0.24   &  y   & 15.52  \\
G08.71-0.41   &  271.6528   &    -21.6213   &   39.64   &  [   28.;   52.] &    4.14   &    0.16   &  y   &  7.41  \\
G11.35+0.80   &  271.8970   &    -18.7276   &   27.59   &  [   12.;   41.] &    1.36   &    0.25   &  n   &  2.43  \\
G10.47+0.03   &  272.1588   &    -19.8638   &   67.05   &  [   56.;   83.] &   12.12   &    0.22   &  n   & 21.68  \\
G10.45-0.02   &  272.1869   &    -19.9100   &   76.06   &  [   66.;   85.] &    2.10   &    0.11   &  n   &  3.75  \\
G10.28-0.12   &  272.1940   &    -20.0978   &   14.29   &  [   -9.;   47.] &    6.67   &    0.25   &  y   & 11.92  \\
G10.29-0.12   &  272.2010   &    -20.0984   &   14.37   &  [    4.;   29.] &    2.84   &    0.12   &  y   &  5.08  \\
G10.34-0.14   &  272.2500   &    -20.0599   &   11.97   &  [   -9.;   39.] &    9.63   &    0.37   &  y   & 17.22  \\
G10.62-0.03   &  272.2860   &    -19.7654   &   64.19   &  [   59.;   76.] &    0.62   &    0.12   &  n   &  1.10  \\
G10.21-0.30   &  272.3350   &    -20.2506   &   12.50   &  [   -9.;   47.] &    3.58   &    0.25   &  y   &  6.40  \\
G10.15-0.34   &  272.3380   &    -20.3244   &    9.81   &  [   -1.;   23.] &    1.36   &    0.12   &  y   &  2.43  \\
G10.21-0.32   &  272.3520   &    -20.2607   &   10.19   &  [  -17.;   25.] &    5.43   &    0.25   &  y   &  9.72  \\
G10.17-0.36A   &  272.3610   &    -20.3175   &   14.02   &  [   -5.;   23.] &    1.48   &    0.12   &  n   &  2.65  \\
G10.17-0.36B   &  272.3650   &    -20.3181   &   15.21   &  [    8.;   21.] &    1.11   &    0.12   &  y   &  1.99  \\
G10.96+0.02   &  272.4140   &    -19.4412   &   21.36   &  [    8.;   35.] &    2.84   &    0.25   &  y   &  5.08  \\
G10.74-0.13   &  272.4400   &    -19.7021   &   29.00   &  [    4.;   61.] &    4.94   &    0.37   &  y   &  8.83  \\
G10.67-0.22   &  272.4920   &    -19.8111   &   29.78   &  [   20.;   47.] &    1.85   &    0.12   &  y   &  3.31  \\
G10.75-0.20   &  272.5130   &    -19.7275   &   31.86   &  [   18.;   35.] &    1.11   &    0.25   &  y   &  1.99  \\
G10.99-0.08   &  272.5270   &    -19.4628   &   29.36   &  [   20.;   37.] &    0.86   &    0.25   &  n   &  1.55  \\
\hline
\end{tabular}
 \tablefoot{The full table is available only in electronic form at the CDS via anonymous ftp to cdsarc.u-strasbg.fr (130.79.125.5) or via http://cdsweb.u-strasbg.fr/cgi-bin/qcat?J/A\&A/. 
 \tablefoottext{a}{Abbreviated source names used for the observations.}
 \tablefoottext{b}{The $v_{\rm lsr}$ of the sources is determined from optically thin tracers in the survey, such as N$_2$H$^+$ (1--0) and H$^{13}$CO$^+$ (1--0).}
 \tablefoottext{c}{The velocity range corresponding to the $FWZP$.}
 \tablefoottext{d}{Error int he integrated intensity of the SiO (2--1) transition.}
 \tablefoottext{e}{The $N(\rm{SiO})$ estimate based on Eq.\,\ref{eq:cdens} and LTE assumption.}
 } 
\end{center}
\end{table*}
%______________________________________________ 


==> SIO_LINEPARAMS_54.tex <==
%______________________________________________
\begin{table*}
\begin{center}
\caption{SiO ($5-4$) line parameters. For some sources the same velocity range was adopted as for the SiO (2--1) line.}\label{tab:table-large-sio54}
\begin{tabular}{lrrrrrrrrrrr}
\hline\hline
Source name\tablefootmark{a}  & Ra      & Dec   & $\Delta v$\tablefootmark{b} &$\int$T$_{mb}\,\rm dv$ & $\sigma_{54}$\tablefootmark{c} & \\
            & J2000 [$^\circ$] & J2000 [$^\circ$]  &  [km/s] &[K km/s]  & [K km/s] & & \\
\hline
G08.68-0.37   &  271.5974   &  -21.6189   &  [    25.;    46.] &    1.31   &    1.27  \\
G08.71-0.41   &  271.6528   &  -21.6213   &  [    36.;    41.] &    0.28   &    0.01  \\
G10.47+0.03   &  272.1588   &  -19.8638   &  [    58.;    81.] &    4.77   &    0.01  \\
G10.45-0.02   &  272.1869   &  -19.9100   &  [    71.;    84.] &    0.27   &    0.01  \\
G10.28-0.12   &  272.1940   &  -20.0978   &  [    -3.;    45.] &    2.14   &    0.22  \\
G10.29-0.12   &  272.2010   &  -20.0984   &  [     6.;    21.] &    0.78   &    0.06  \\
G10.34-0.14   &  272.2500   &  -20.0599   &  [    -7.;    49.] &    3.85   &    0.13  \\
G10.21-0.32   &  272.3520   &  -20.2607   &  [   -17.;    25.] &    0.75   &    0.18  \\
G10.74-0.13   &  272.4400   &  -19.7021   &  [    16.;    32.] &    0.59   &    0.08  \\
G10.62-0.38   &  272.6193   &  -19.9300   &  [   -17.;    12.] &    8.79   &    0.07  \\
G12.42+0.51   &  272.7110   &  -17.9292   &  [     2.;    31.] &    0.37   &    0.07  \\
G11.08-0.53   &  272.9950   &  -19.6004   &  [    23.;    46.] &    1.17   &    0.10  \\
G11.90-0.14   &  273.0460   &  -18.6918   &  [    38.;    46.] &    0.16   &    0.19  \\
G12.20-0.03   &  273.0980   &  -18.3801   &  [    38.;    58.] &    1.38   &    0.19  \\
G12.21-0.10   &  273.1650   &  -18.4040   &  [     8.;    43.] &    1.84   &    0.01  \\
G12.90-0.03   &  273.4500   &  -17.7595   &  [    34.;    83.] &    1.48   &    0.10  \\
G12.68-0.18   &  273.4760   &  -18.0294   &  [    40.;    63.] &    0.31   &    0.11  \\
G11.92-0.61   &  273.4920   &  -18.9052   &  [    10.;    57.] &    8.80   &    0.10  \\
G11.94-0.61   &  273.5030   &  -18.8899   &  [    28.;    51.] &    0.50   &    0.08  \\
\hline
\end{tabular}
 \tablefoot{The full table is available only in electronic form at the CDS via anonymous ftp to cdsarc.u-strasbg.fr (130.79.125.5) or via http://cdsweb.u-strasbg.fr/cgi-bin/qcat?J/A\&A/.
 \tablefoottext{a}{Abbreviated source names used for the observations.}
 \tablefoottext{b}{The velocity range corresponding to the $FWZP$ determined from the SiO (2--1) observartions.}
 \tablefoottext{c}{Error in the integrated intensity of the SiO (5--4) transition.}}
\end{center}
\end{table*}
%______________________________________________ 

